How close are cone singularities on a random flat surface?

We study the shortest geodesics on flat cone spheres, i.e. flat metrics on the sphere with conical singularities. The length of the shortest geodesic between two singular points can be treated as a function on the moduli space of flat cone spheres with prescribed angle defects. We prove a recurrent relation on the distribution of this function with respect to Thurston's volume form on the moduli space.

==> _think.tex <==

The central object of study is a flat cone sphere.
The space of flat cone spheres...



















For $n=1$ it holds
$s = \frac{\sin\frac{\phi_1}{2}\sin\frac{\phi_2}{2}}{2\sin\frac{\alpha_1}{2}}$, therefore,
$f(\phi, \alpha, s) = \delta(s-\frac{\sin\frac{\phi_1}{2}\sin\frac{\phi_2}{2}}{2\sin\frac{\alpha_1}{2}})$.


For $n=2$ the support of $s$ is $[....]$
